Rethinking Query-based Transformer for Continual Image Segmentation

Class-incremental/Continual image segmentation (CIS) aims to train an image segmenter in stages, where the set of available categories differs at each stage. To leverage the built-in objectness of query-based transformers, which mitigates catastrophic forgetting of mask proposals, current methods often decouple mask generation from the continual learning process. This study, however, identifies two key issues with decoupled frameworks: loss of plasticity and heavy reliance on input data order. To address these, we conduct an in-depth investigation of the built-in objectness and find that highly aggregated image features provide a shortcut for queries to generate masks through simple feature alignment. Based on this, we propose SimCIS, a simple yet powerful baseline for CIS. Its core idea is to directly select image features for query assignment, ensuring "perfect alignment" to preserve objectness, while simultaneously allowing queries to select new classes to promote plasticity. To further combat catastrophic forgetting of categories, we introduce cross-stage consistency in selection and an innovative "visual query"-based replay mechanism. Experiments demonstrate that SimCIS consistently outperforms state-of-the-art methods across various segmentation tasks, settings, splits, and input data orders. All models and codes will be made publicly available at https://github.com/SooLab/SimCIS.

==> sec/tab/rebuttal_orders.tex <==

\begin{table*}[b]
\centering
  \begin{adjustbox}{max width=0.95\linewidth}
    \begin{tabular}{c|ccccccccc|ccccccccc}
        \toprule
         \multirow{3}*{Random ID} & \multicolumn{9}{c}{Our SimCIS} & \multicolumn{9}{c}{ECLIPSE} \\
          \multirow{3}*{} & \multicolumn{3}{c}{1-100} & \multicolumn{3}{c}{101-150}
         & \multicolumn{3}{c}{all} & \multicolumn{3}{c}{1-100} & \multicolumn{3}{c}{101-150}
         & \multicolumn{3}{c}{all}\\
           \multirow{3}*{} & \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ} & \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ}& \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ} & \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ} & \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ} & \textit{PQ}~~ & ~~\textit{SQ} & \textit{RQ}\\
        \midrule
        
         1~~~& 41.2                   &                        &                        & 28.9                   &                        &                        & 37.1                   & 75.6                       &44.1                         & 33.4                   & 76.2                   & 40.1                   & 20.4                   & 56.3                   & 24.8                   & 29.1                   & 69.6                   & 35.0                   \\
         2~~~& 42.2                   &                        &                        & 30.2                   &                        &                        & 38.2                   & 75.8                    & 45.5                       & 32.1                   & 71.4                   & 38.4                   & 22.9                   & 65.0                   & 27.8                   & 29.1                   & 69.3                   & 35.0                   \\
         
         3~~~& 41.1                   &                        &                        & 29.8                   &                        &                        & 37.3                   &  76.0                      & 44.6                   & 32.2                   & 72.2                   & 38.0                   & 23.3                   & 67.0                   & 28.5                   & 29.3                   & 68.4                   & 35.5                   \\
         
         4~~~& 42.2                   &                        &                        & 29.6                   &                        &                        & 38.0                   & 77.9                     & 45.3                    & 30.4                   & 73.1                   & 37.1                   & 18.0                   & 58.3                   & 21.4                   & 26.3                   & 68.2                   & 31.8                   \\
         
         5~~~& 41.2                   &                        &                        & 30.5                   &                        &                        & 37.6                   & 78.5                     & 44.8                     & 32.2                   & 76.1                   & 41.0                   & 22.8                   & 57.2                   & 23.0                   & 29.1                   & 69.8                   & 35.0                   \\
         
         6~~~& 41.7                   &                        &                        & 27.5                   &                        &                        & 37.0                   &  75.1                   & 44.1                     & 28.5                   & 67.4                   & 34.4                   & 24.3                   & 61.0                   & 28.9                   & 27.1                   & 65.3                   & 32.5                   \\
         
         7~~~ & 41.9                   &                        &                        & 28.8                   &                        &                        & 37.6                   &                        &                         & 34.3                   & 76.2                   & 41.0                   & 18.8                   & 57.0                   & 23.1                   & 29.2                   & 70.0                   & 35.0                   \\
         
         8~~~& 40.0                   &                        &                        & 29.9                   &                        &                        & 36.6                   & 76.0                       & 44.6                        & 30.4                   & 74.7                   & 37.0                   & 22.7                   & 63.0                   & 27.2                   & 27.9                   & 70.8                   & 33.8                   \\
         
         9~~~& 42.0                   &                        &                        & 28.7                   &                        &                        & 37.6                   &                        &                         & 32.7                   & 75.3                   & 39.0                   & 22.2                   & 64.9                   & 26.9                   & 29.2                   & 71.9                   & 35.0                   \\
         
         10\dag& 39.1                   &                        &                        & 33.8                   &                        &                        & 37.4                   & 77.3                       &  44.5                       & 11.3                   & 36.5                   & 14.1                   & 0.0                    & 0.0                    & 0.0                    & 7.6                    & 24.3                   & 9.4                    \\
         \midrule
         Origin & 42.2                   &                        &                        & 30.1                   &                        &                        & 38.1                   &                        &                         & 41.4                   & 78.4                   & 49.4                   & 18.8                   & 71.0                   & 23.0                   & 33.9                   & 75.9                   & 40.6                  \\
         \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Continual Panoptic Segmentation with 10 random order}  on the ADE20K 100-5 continual panoptic segmentation scenario. \dag{ }means descending order. Origin means original ascending order. Follow ECLIPSE\cite{(eclipse)kim2024eclipse}, we provide segmentation quality(\textit{SQ}) and recognition quality(\textit{RQ}) to further illustrate the effectiveness of our SimCIS.}
    \label{tab:rebut_unorder}
\end{table*}
